Optimus: Organizing Sentences via Pre-trained Modeling of a Latent Space

When trained effectively, the Variational Autoencoder (VAE) can be both a powerful generative model and an effective representation learning framework for natural language. In this paper, we propose the first large-scale language VAE model, Optimus. A universal latent embedding space for sentences is first pre-trained on large text corpus, and then fine-tuned for various language generation and understanding tasks. Compared with GPT-2, Optimus enables guided language generation from an abstract level using the latent vectors. Compared with BERT, Optimus can generalize better on low-resource language understanding tasks due to the smooth latent space structure. Extensive experimental results on a wide range of language tasks demonstrate the effectiveness of Optimus. It achieves new state-of-the-art on VAE language modeling benchmarks. We hope that our first pre-trained big VAE language model itself and results can help the NLP community renew the interests of deep generative models in the era of large-scale pre-training, and make these principled methods more practical.

==> subtex/understanding.tex <==


\subsection{Low-resource Language Understanding} %  and Discussion

\paragraph{Sentiment classification on Yelp dataset.} We consider the Yelp dataset collected in~\cite{shen2017style}. 
It contains 444K training sentences, and we use separated datasets of 10K sentences for validation/testing, respectively. 
A linear classifier is added on the feature of $\mathtt{[CLS]}$ token. A various number of samples are randomly chosen for training, ranging from 1 to 10K per class. 10 runs are used when the available training samples are rare. 
100 training epochs are used in each setting. 
Two schemes are used to leverage pre-trained models: (1) {\it Fine-tuning}, where both the pre-trained model and the linear classifier are updated; (2) {\it Feature-based}, where pre-trained model weights are frozen to provide embeddings for the update of the linear classifier. The results are shown in Figure~\ref{fig:ssl_yel_acc}. 
%
When pre-trained models are used to provide sentence embeddings, the proposed \short{}  consistently outperforms BERT. It demonstrated that the latent structures learned by \short{}  is more separated, and help generalize better. When the entire network is fine-tuning, \short{}  can adapt faster than BERT,  when the available number of training samples is small. The two methods perform quite similarly when more training data is provided. This is because the pre-trained model size is much larger than the linear classifier, which the performance is largely is dominated by main networks in training.


\paragraph{Visualization of the latent space.}
%
We use tSNE~\cite{maaten2008visualizing}  to visualize the learned feature on a 2D map. The validation set of Yelp is used to extract the latent features. \short{}  and BERT
Compared with BERT, \short{}  learns a smoother space and more structured latent patterns, which explains why \short{}  can yield better classification performance and faster adaptation. 


\paragraph{GLUE.} We further consider GLUE benchmark, and show the results on the validation set in Table~\ref{tab:compare_glue}. With the feature-based scheme, \short{}  yields higher performance than BERT, especially on the large datasets. When the full models are fine-tuned, the two methods perform quite similarly. 



\begin{figure}[t!]%\vspace{-25pt}
	\vspace{-0mm}\centering
	\includegraphics[width=6.75cm]{figs/yelp_ssl.pdf}
	\vspace{-3mm}
	\caption{\small Testing accuracy with a various number of training samples on the Yelp dataset.}
	\vspace{2mm}
	\label{fig:ssl_yel_acc}
\end{figure}
%


\begin{figure*}[t!]%\vspace{-25pt}
	\vspace{-0mm}\centering
	\begin{tabular}{cc}
	    \hspace{-3mm}		
		\includegraphics[height=3.9cm]{figs/latent_vis/yelp_vae_feature_vis.pdf} &
		\includegraphics[height=3.9cm]{figs/latent_vis/yelp_bert_feature_vis.pdf} \\
		\hspace{-3mm}		
		(a) \short{}  &
		(b) BERT
	\end{tabular}
	\vspace{-0mm}
	\caption{Comparison of tSNE visualization for the self-supervised feature learning results. The colors indicate different labels.}
	\vspace{-0mm}
	\label{fig:tsne_latent_supp}
\end{figure*}


\begin{table*}[t!]
    \centering
  \vspace{-0mm}
  \begin{adjustbox}{scale=0.95,tabular=c|c|cccccccccc}
    \toprule
     \multicolumn{2}{ c|}{System}
     &
     MNLI & QQP & QNLI & SST-2 & CoLA & STS-B & MRPC & RTE  & WNLI & {\bf Average} \\
     \multicolumn{2}{ c|}{Dataset size}
     &
     392k & 363k & 108k & 67k & 8.5k & 5.7k & 3.5k & 2.5k  & 634 &  \\     
    \midrule 
    \multirow{2}{*}{Feature-based}
    & BERT & 0.414 & 0.146 & 0.673 & 0.731 & 0.000 & 0.608 & 0.812 & 0.527 & 0.563 & 0.497 \\
    & \short{}  &  {\color{blue}  0.468}  & {\color{blue}  0.662} & {\color{blue}  0.720} & {\color{blue}  0.789} & 0.000 & 0.518 & 0.809 & {\color{blue}  0.531 } & 0.563 & \textbf{\color{blue}  0.562} \\ 
    \midrule 
    \multirow{2}{*}{Fine-tuning}
    & BERT & 0.835 & 0.909 & 0.912 & 0.923 & 0.598 & 0.886 & 0.868 & 0.700 & 0.507
 & 0.793 \\
    & \short{}  & 0.834 & 0.909 & 0.908 & 0.924 & 0.573 & 0.888 & 0.873 & 0.697 & 0.563 & \textbf{\color{blue}  0.797} \\ 
  \bottomrule
\end{adjustbox}
\vspace{-0mm}
  \caption{\small Comparison on the validation set of GLUE. F1 scores are reported for QQP and MRPC, Spearman correlations are reported for STS-B, and accuracy scores are reported for the other tasks.}
  \label{tab:compare_glue}
\vspace{-0mm}
\end{table*}

